Harvesting Expert-Parallel Bubbles for Fine-Tuning

GPUs are expensive, yet latency-critical large language model (LLM) inference leaves part of them idle. Colocation reclaims this capacity by running best-effort work, such as fine-tuning, alongside serving. Many leading LLMs now use a Mixture-of-Experts (MoE) architecture, which adds a new source of idle time. Under expert parallelism, MoE experts are spread across GPUs, and because the router sends uneven numbers of tokens to each GPU, lightly loaded GPUs wait for the most loaded one. Even after applying load balancing solutions, such bubbles still take 8--13% of prefill time. We present BubbleTea, the first colocation system that leverages expert-parallel bubbles for fine-tuning. Unlike existing colocation systems, which make one scheduling decision for all GPUs per forward pass, BubbleTea predicts each GPU's bubble at every layer from the router's token assignment, and fills it with short chunks of fine-tuning work that reuse the weights already loaded for serving. We also introduce compiler passes that automatically derive these chunks from the served LLM as-is, without porting each model architecture to a separate training engine. Our evaluation on three MoE models, served on four A100 GPUs, shows that fine-tuning throughput with BubbleTea is 1.9--6.2$\times$ faster than with LLMStation, a state-of-the-art colocation system. BubbleTea keeps p90 inference latency within 10% of serving alone in 50 of 63 workloads, compared to 44 for LLMStation. On bursty production traces, BubbleTea trains 3.3$\times$ faster than LLMStation and 14$\times$ faster than a stock trainer colocated under CUDA MPS, with p90 inference latency staying within 7% of serving alone.

==> plots/e2e_latency_defs.tex <==
\pgfplotstableread[col sep=comma]{plots/CSVs/e2e_latency.csv}\lattable
\protected\def\latcliplabel{%
  \pgfkeys{/pgf/fpu=true, /pgf/fpu/output format=fixed}%
  \pgfmathparse{\pgfplotspointmeta}\let\latv\pgfmathresult
  \pgfkeys{/pgf/fpu=false}%
  \ifdim\latv pt>2pt
    \ifdim\latv pt<10pt
      \pgfmathprintnumber[fixed, fixed zerofill, precision=1]{\latv}%
    \else
      \pgfmathprintnumber[fixed, precision=0]{\latv}%
    \fi$\times$%
  \fi}
\newcommand{\latpanel}[3]{%
  \nextgroupplot[#3]
  \addplot[fill=sysLLMStation, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax},
    point meta=\thisrow{llmstation_#2}, label left]
    table[x expr=\coordindex, y=llmstation_#2]{\lattable};
  \addplot[fill=sysNaive40, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax},
    point meta=\thisrow{naive40_#2}, naive label]
    table[x expr=\coordindex, y=naive40_#2]{\lattable};
  \addplot[fill=sysBubbleTea, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax},
    point meta=\thisrow{bubbletea_#2}, label right]
    table[x expr=\coordindex, y=bubbletea_#2]{\lattable};
  \latrefs
}
\newcommand{\latrefs}{%
  \draw[thin, densely dashed] ({rel axis cs:0,0} |- {axis cs:0,1})
    -- ({rel axis cs:1,0} |- {axis cs:0,1});
  \draw[thin, densely dotted] ({rel axis cs:0,0} |- {axis cs:0,1.1})
    -- ({rel axis cs:1,0} |- {axis cs:0,1.1});}
\newcommand{\latlegend}{%
  \addlegendentry{LLMStation}
  \addlegendentry{\Uncoord (40\% cap)}
  \addlegendentry{\sys{}}}
\protected\def\latticklabel{\pgfmathtruncatemacro{\latrow}{\tick}%
  \pgfplotstablegetelem{\latrow}{req_per_s}\of\lattable
  \pgfmathprintnumber[precision=2]{\pgfplotsretval}}
\pgfplotsset{latgrid/.style={
      bar plot,
      typeset ticklabels with strut,
      ybar=0pt, /pgf/bar width=4pt,
      enlarge x limits=0.25,
      title style={yshift=-3pt},
      ymin=0.6, ymax=2, ytick={1,1.5,2},
      restrict y to domain*=0:2,
      nodes near coords={\latcliplabel},
      every node near coord/.append style={font=\tiny, rotate=90,
        inner xsep=0.5pt, inner ysep=2.5pt},
      label left/.style={every node near coord/.append style={
        anchor=south east}},
      label right/.style={every node near coord/.append style={
        anchor=north east}},
      naive label/.style={label left},
      xticklabel={\latticklabel},
      ylabel style={align=center},
}}


==> plots/eplb_defs.tex <==
\tikzset{eplb hatch/.style={postaction={pattern=north east lines,
  pattern color=black!50}}}
\newcommand{\epftbar}[3]{%
  \addplot[forget plot, fill=white, draw=black, densely dashed,
    /pgf/bar shift=#2,
    point meta={(\thisrow{ft_#1_bubbletea}/\thisrow{ft_#1_base}-1)*100},
    nodes near coords={\pgfmathprintnumber[fixed, precision=0,
      print sign]{\pgfplotspointmeta}\%},
    every node near coord/.append style={font=\tiny, inner sep=1pt,
      solid, rotate=90, anchor=west}]
    table[x expr=\coordindex,
      y expr={max(\thisrow{ft_#1_base}, \thisrow{ft_#1_bubbletea})}]{\eptable};
  \addplot[forget plot, fill=ladderE, draw=black, /pgf/bar shift=#2, #3]
    table[x expr=\coordindex, y=ft_#1_bubbletea]{\eptable};
  \addplot[forget plot, fill=ladderB, draw=black, /pgf/bar shift=#2, #3]
    table[x expr=\coordindex,
      y expr={min(\thisrow{ft_#1_base}, \thisrow{ft_#1_bubbletea})}]{\eptable};
}
\newcommand{\eplatbars}[1]{%
  \addplot[forget plot, fill=pastel8, draw=black, /pgf/bar shift=-6pt]
    table[x expr=\coordindex, y=#1_alone_noeplb]{\eptable};
  \addplot[forget plot, fill=pastel8, draw=black, eplb hatch,
    /pgf/bar shift=0pt]
    table[x expr=\coordindex, y expr=1]{\eptable};
  \addplot[forget plot, fill=ladderE, draw=black, eplb hatch,
    /pgf/bar shift=6pt]
    table[x expr=\coordindex, y=#1_bubbletea_eplb]{\eptable};
  \draw[thin, densely dashed] ({rel axis cs:0,0} |- {axis cs:0,1})
    -- ({rel axis cs:1,0} |- {axis cs:0,1});
  \draw[thin, densely dotted] ({rel axis cs:0,0} |- {axis cs:0,1.1})
    -- ({rel axis cs:1,0} |- {axis cs:0,1.1});
}
\newcommand{\epsep}{%
  \draw[thin, black!40] ({axis cs:2.5,0} |- {rel axis cs:0,0})
    -- ({axis cs:2.5,0} |- {rel axis cs:0,1});}
\newcommand{\epgroup}[2]{%
  \node[anchor=north, font=\sffamily\footnotesize, yshift=-11pt]
    at ({axis cs:#1,0} |- {rel axis cs:0,0}) {#2};}
\protected\def\epticklabel{\pgfmathtruncatemacro{\eprow}{\tick}%
  \pgfplotstablegetelem{\eprow}{prompt_tokens}\of\eptable
  \edef\epk{\the\numexpr\pgfplotsretval/1024\relax}%
  \pgfplotstablegetelem{\eprow}{req_per_s}\of\eptable
  \epk k @ \pgfmathprintnumber[precision=4]{\pgfplotsretval}}


==> plots/ft_throughput_defs.tex <==
\pgfplotstableread[col sep=comma]{plots/CSVs/ft_throughput.csv}\fttable
\newcommand{\ftpanel}[2]{%
  \nextgroupplot[#2]
  \addplot[fill=sysLLMStation, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=llmstation]{\fttable};
  \addplot[fill=sysNaive40, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=naive40]{\fttable};
  \addplot[fill=sysBubbleTea, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax},
    point meta=\thisrow{bubbletea_over_llmstation},
    nodes near coords={\pgfmathprintnumber[fixed, fixed zerofill,
      precision=1]{\pgfplotspointmeta}$\times$},
    visualization depends on={\thisrow{label_lift} \as \ftlift},
    every node near coord/.append style={font=\tiny,
      text=black, inner sep=1pt,
      shift={(axis direction cs:0,\ftlift)}}]
    table[x expr=\coordindex, y=bubbletea]{\fttable};
}
\protected\def\ftticklabel{\pgfmathtruncatemacro{\ftrow}{\tick}%
  \pgfplotstablegetelem{\ftrow}{req_per_s}\of\fttable
  \pgfmathprintnumber[precision=2]{\pgfplotsretval}}
\newcommand{\ftlegend}{%
  \addlegendentry{LLMStation}
  \addlegendentry{\Uncoord (40\% cap)}
  \addlegendentry{\sys{}}}


==> plots/latency_ablation_defs.tex <==
\pgfplotstableread[col sep=comma]{plots/CSVs/latency_ablation.csv}\labtable
\protected\def\labcliplabel{%
  \pgfkeys{/pgf/fpu=true, /pgf/fpu/output format=fixed}%
  \pgfmathparse{\pgfplotspointmeta}\let\labv\pgfmathresult
  \pgfkeys{/pgf/fpu=false}%
  \ifdim\labv pt>2pt
    \pgfmathprintnumber[fixed, fixed zerofill, precision=1]{\labv}$\times$%
  \fi}
\newcommand{\labpanel}[3]{%
  \nextgroupplot[#3]
  \addplot[fill=ladderB, draw=black, point meta=\thisrow{b_#2},
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=b_#2]{\labtable};
  \addplot[fill=ladderC, draw=black, point meta=\thisrow{c_#2},
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=c_#2]{\labtable};
  \addplot[fill=ladderD, draw=black, point meta=\thisrow{d_#2},
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=d_#2]{\labtable};
  \addplot[fill=ladderE, draw=black, point meta=\thisrow{e_#2},
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=e_#2]{\labtable};
}
\newcommand{\labreflines}{%
  \draw[thin, densely dashed] ({rel axis cs:0,0} |- {axis cs:0,1})
    -- ({rel axis cs:1,0} |- {axis cs:0,1});
  \draw[thin, densely dotted] ({rel axis cs:0,0} |- {axis cs:0,1.1})
    -- ({rel axis cs:1,0} |- {axis cs:0,1.1});
}
\protected\def\labticklabel{\pgfmathtruncatemacro{\labrow}{\tick}%
  \pgfplotstablegetelem{\labrow}{req_per_s}\of\labtable
  \pgfmathprintnumber[precision=4]{\pgfplotsretval}}
\pgfplotsset{
  labft/.style={ymax=6, ytick={0,2,4,6}},
  labratio/.style={ymin=0.6, ymax=2, ytick={1,1.5,2},
    restrict y to domain*=0:2,
    nodes near coords={\labcliplabel},
    every node near coord/.append style={font=\tiny, rotate=90,
      anchor=south east, inner xsep=0.5pt, inner ysep=2.5pt}},
}
\newcommand{\lablegend}{%
  \addlegendentry{\textbf{\textsc{Tea}}}
  \addlegendentry{Unconstrained scheduling}
  \addlegendentry{Constrained scheduling}
  \addlegendentry{\sys{}}}


==> plots/naive_sweep_defs.tex <==
\input{plots/e2e_latency_defs}%
\pgfplotstableread[col sep=comma]{plots/CSVs/naive_sweep.csv}\nstable
\newcommand{\nspanel}[3]{%
  \nextgroupplot[#3]
  \addplot[fill=sysNaiveCap, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax},
    point meta=\thisrow{naive6#2}, label left,
    visualization depends on={\thisrow{naive40#2} \as \nsforty},
    every node near coord/.append style={/utils/exec={%
      \ifdim\nsforty pt>2pt \pgfkeysalso{/tikz/yshift=5pt}\fi}}]
    table[x expr=\coordindex, y=naive6#2]{\nstable};
  \addplot[fill=sysNaive40, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax},
    point meta=\thisrow{naive40#2}, label left]
    table[x expr=\coordindex, y=naive40#2]{\nstable};
  \addplot[fill=sysNaive, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax},
    point meta=\thisrow{naivenone#2},
    visualization depends on={\thisrow{naive40#2} \as \nsforty},
    visualization depends on={\thisrow{naive6#2} \as \nssix},
    every node near coord/.append style={/utils/exec={%
      \ifdim\nsforty pt>1.6pt \pgfkeysalso{/tikz/anchor=north east}%
      \else\ifdim\nssix pt>2pt \pgfkeysalso{/tikz/anchor=north east}%
      \else \pgfkeysalso{/tikz/anchor=south east}\fi\fi}}]
    table[x expr=\coordindex, y=naivenone#2]{\nstable};
}
\protected\def\nsticklabel{\pgfmathtruncatemacro{\nsrow}{\tick}%
  \pgfplotstablegetelem{\nsrow}{req_per_s}\of\nstable
  \pgfmathprintnumber[precision=2]{\pgfplotsretval}}
\newcommand{\nslegend}{%
  \addlegendentry{\Uncoord (6\% cap)}
  \addlegendentry{\Uncoord (40\% cap)}
  \addlegendentry{\Uncoord (no cap)}}


==> plots/sources_defs.tex <==
\pgfplotstableread[col sep=comma]{plots/CSVs/sources.csv}\srctable
\newcommand{\srcpanel}[2]{%
  \nextgroupplot[#2]
  \addplot[fill=ladderA, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=a_plain]{\srctable};
  \addplot[fill=ladderB, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=b_second_chain]{\srctable};
  \addplot[fill=ladderE, draw=black,
    select coords between index={#1}{\numexpr#1+2\relax}]
    table[x expr=\coordindex, y=e_bubbletea]{\srctable};
}
\protected\def\srcticklabel{\pgfmathtruncatemacro{\srcrow}{\tick}%
  \pgfplotstablegetelem{\srcrow}{req_per_s}\of\srctable
  \pgfmathprintnumber[precision=4]{\pgfplotsretval}}

